CTD: Fast, Accurate, and Interpretable Method for Static and Dynamic Tensor Decompositions

How can we find patterns and anomalies in a tensor, or multi-dimensional array, in an efficient and directly interpretable way? How can we do this in an online environment, where a new tensor arrives each time step? Finding patterns and anomalies in a tensor is a crucial problem with many applications, including building safety monitoring, patient health monitoring, cyber security, terrorist detection, and fake user detection in social networks. Standard PARAFAC and Tucker decomposition results are not directly interpretable. Although a few sampling-based methods have previously been proposed towards better interpretability, they need to be made faster, more memory efficient, and more accurate. In this paper, we propose CTD, a fast, accurate, and directly interpretable tensor decomposition method based on sampling. CTD-S, the static version of CTD, provably guarantees a high accuracy that is 17 ~ 83x more accurate than that of the state-of-the-art method. Also, CTD-S is made 5 ~ 86x faster, and 7 ~ 12x more memory-efficient than the state-of-the-art method by removing redundancy. CTD-D, the dynamic version of CTD, is the first interpretable dynamic tensor decomposition method ever proposed. Also, it is made 2 ~ 3x faster than already fast CTD-S by exploiting factors at previous time step and by reordering operations. With CTD, we demonstrate how the results can be effectively interpreted in the online distributed denial of service (DDoS) attack detection.

==> 060related.tex <==
In this section, we describe existing sampling-based tensor decomposition methods. Drineas et al. proposed ApproxTensorSVD \cite{drineas2007randomized}. ApproxTensorSVD has resulting factor matrix on each mode while CTD or tensor-CUR has a factor matrix for only one mode. ApproxTensorSVD performs matricization, samples fibers on all mode, and then joins them in the form of Tucker decomposition, the $n$-dimensional extension of SVD. Caiafa et al. \cite{caiafa2010generalizing} proposed FBTD (fiber-based tensor decomposition). FBTD is also in the form of Tucker decomposition as ApproxTensorSVD, but it differs from ApproxTensorSVD in the way of sampling fibers. We limit our discussion on sampling-based tensor decomposition to the mode-$\alpha$ LR tensor decomposition in Definition \ref{def:LR tensor decomposition}, which performs on only one specified mode $\alpha$. This is because Tucker-type sampling-based tensor decomposition method requires long running time since it performs computation for all modes. Thus it is not applicable for practical use and is also difficult to devise its dynamic version. In addition, there is no known existing sampling-based dynamic tensor decomposition method so far, which incrementally updates its factors on the online environment. \revision{Sampling-based methods : \cite{chang2015incremental,liu2014incremental}} 
